Human Movement Forecasting with Loose Clothing

Human motion prediction and trajectory forecasting are essential in human motion analysis. Nowadays, sensors can be seamlessly integrated into clothing using cutting-edge electronic textile (e-textile) technology, allowing long-term recording of human movements outside the laboratory. Motivated by the recent findings that clothing-attached sensors can achieve higher activity recognition accuracy than body-attached sensors. This work investigates the performance of human motion prediction using clothing-attached sensors compared with body-attached sensors. It reports experiments in which statistical models learnt from the movement of loose clothing are used to predict motion patterns of the body of robotically simulated and real human behaviours. Counterintuitively, the results show that fabric-attached sensors can have better motion prediction performance than rigid-attached sensors. Specifically, The fabric-attached sensor can improve the accuracy up to 40% and requires up to 80% less duration of the past trajectory to achieve high prediction accuracy (i.e., 95%) compared to the rigid-attached sensor.

==> comments.tex <==
% define simple todo command
%\usepackage{lineno}
\usepackage[normalem]{ulem}                                        % for striking text out
\usepackage{marginnote}
\setlength{\marginparwidth}{1.75cm}
\setlength{\marginparsep}{.1mm}
\usepackage[textwidth=\marginparwidth,colorinlistoftodos]{todonotes}
\providecommand{\tinytodo}[2][]
{\todo[caption={#2}, size=\small, #1]{\renewcommand{\baselinestretch}{0.6}\selectfont#2\par}}

% define colours for to-dos
\colorlet{jb}{red}
\colorlet{mh}{red}
\providecommand{\commentcolourcode}{Comments colour code: 
{\color{mh}MH}} 
\providecommand  {\colorsout}[1]{\bgroup\markoverwith{\textcolor{#1}{\rule[0.5ex]{2pt}{0.4pt}}}\ULon} % define coloured strike out
\providecommand{\atMH} {{\color{mh}@MH}}
\providecommand{\atJB} {{\color{jb}@JB}}

\providecommand  {\done}   [1]{\sout{#1}}
\providecommand  {\edit}   [3]{\colorsout{#3}{#1}{\color{#3}{#2}}}
\providecommand  {\nomment}[2]{\tinytodo[color=white,nolist,linecolor=#2,bordercolor=white,noinline]{\protect{\scriptsize\color{#2}#1}}}
\providecommand  {\note}[2]{\tinytodo[color=white,linecolor=#2,bordercolor=white,noinline]{\protect{\scriptsize\color{#2}#1}}}
%\providecommand  {\at}     [1]{\textcolor{#2}{@#2}}

\providecommand{\cn}{\note{Citation needed.}{mh}} % shortcut commenting commands


\providecommand{\makecomments}{%
\section*{Usage notes}~\\%[1ex]
\noindent Use \texttt{\textbackslash note\{your comment\}\{your initials\}} to add comments/to dos. For example,
\underline{J}oe \underline{B}loggs adds comments using \texttt{\textbackslash note\{Comment.\}\{jb\}}.\nomment{These comments will appear as margin notes. They will also appear in the todo list on the first page.}{jb} \\[2ex]
%\noindent Optionally, use \texttt{\textbackslash atInitials} to address your comment to someone (\eg \texttt{\textbackslash note\{\textbackslash atJB: Please fix this.\}\{mh\}}).\\[2ex]
You can mark a comment as resolved using \texttt{\textbackslash done\{Comment text.\}}, (\eg \texttt{\textbackslash note\{\textbackslash done\{\textbackslash atJB: Please fix this.\}\}\{mh\}}). It will then be formatted like this: \done{\atJB: Please fix this.}.\\[2ex]
\commentcolourcode\\[1ex]
\printacronyms~\\[2ex]% if using glossaries package to manage acronyms, print them
\listoftodos~\\[2ex]
\clearpage\setcounter{page}{1}
%\linenumbers%
}

\providecommand{\makenotes}{\clearpage\appendix\input{notes}}%

\providecommand{\makefinal}{%
\renewcommand{\makecomments}{}\renewcommand{\makenotes}{}\renewcommand{\note}[1]{}\renewcommand{\done}[1]{}\renewcommand{\edit}[3]{\#2}\renewcommand{\comment}[2]{}%
}


==> gmr.tex <==
\subsection{\gls{gmr}}
Given sensor reading from four sensors, sensors were recorded rigid and fabric movement with $30$ sequences. All sequence was synchronised. Each category (\ie low and high frequency) of data were treated as \gls{gmm}. \gls{em} algorithm is used to estimate \gls{pdf} of it. 
The initial parameters of each \gls{gmm} is using k-means clustering algorithm. We will denote the block decomposition of a data point from sensors reading $\xr_{t}$ at time step $t$, and the center $\mu_{i}$ and covariance $\Sigma_{i}$ of the $i$-th Gaussian in the \gls{gmm}.
\begin{equation}
x_{i} = 
\begin{bmatrix}
    t_{i}   \\
    \xr_{i}
\end{bmatrix},
\mu_{i}=
\begin{bmatrix}
    \mu_{t_{i}}   \\
    \mu_{\xr_{i}}
\end{bmatrix},
\Sigma_{i}=
\begin{bmatrix}
    \Sigma\{t_{i},t_{i}\} & \Sigma\{t_{i},\xr_{i}\} \\
    \Sigma\{\xr_{i},t_{i}\} &  \Sigma\{\xr_{i},\xr_{i}\}
\end{bmatrix}.
\end{equation}
The \gls{pdf} is given by
\begin{equation}
f(x|\theta) = \sum_{i=1}^{m}\alpha_{i}\mathcal N(\mu_{i},\Sigma_{i}),
\end{equation}
where $m$ is the number of gaussian components and $\alpha_{i}$ is the weights of each $i$-th Gaussian component.

\gls{kl} between \gls{gmm}s has no closed form to be computed but it can be estimated in different approaches \cite{4218101} \cite{durrieu2012lower}. We use the variational approximation as it has a good balance between computation time and accuracy \cite{cui2015comparison}. 

\gls{kl} divergence between different movements from sensors reading $\D(x^{\w1}||x^{\w2})$ could be estimated by
\begin{equation}
\D(x^{\w1}||x^{\w2}) = \sum_{i=1}^{M}\alpha_{i}^{\w1}log\frac{\sum_{i=1}^{M}\alpha_{i}^{\w1}\exp({-\D(x^{\w1}_{i}||x^{\w1}_{i'})})}{\sum_{j=1}^{N}\alpha_{j}^{\w2}\exp({-\D(x^{\w1}_{i}||x^{\w2}_{j})})},
\end{equation}
where $M$ and $N$ are the number of Gaussian components for low and high frequency respectively and $x^{\w1}_{i}$ and $x^{\w2}_{j}$ are single Gaussian components. (\ie $x^{\w1}_{i} = \mathcal N(\mu_{i}^{\w1},\Sigma_{i}^{\w1})$ $x^{\w2}_{j} = \mathcal N(\mu_{j}^{\w2},\Sigma_{j}^{\w2})$).

\gls{kl} divergence $\D(x^{\w1}_{i}||x^{\w2}_{j})$ between two Gaussian functions has a closed-form equation,
\begin{equation}
\begin{split}
    \D(x^{\w1}_{i}||x^{\w2}_{j})=&\frac{1}{2}[\log\frac{\Sigma_{x^{\w2}_{j}}}{\Sigma_{x^{\w1}_{i}}}+\DeclareMathOperator{\Tr}{Tr}[\Sigma^{-1}_{x^{\w2}_{j}}\Sigma_{x^{\w1}_{i}}]-d\\
    &+(\mu_{x^{\w1}_{i}}-\mu_{x^{\w2}_{j}})^\T\Sigma^{-1}_{x^{\w2}_{j}}(\mu_{x^{\w1}_{i}}-\mu_{x^{\w2}_{j}})].
    \end{split}
\end{equation}
where $d$ is dimension. 
\gls{gmr} is used to estimate the most possible sequence from multiple sequences. Consecutive temporal values $x^{*}$ are used as query points and the corresponding spatial values $y$ and $\sigma$ are estimated through regression. 
%For each $i$-th Gaussian component, the conditional expectation $\xi_{s,i}$ given $\xi_{t}$, and the estimated conditional covariance of  $\xi_{s,i}$ given $\xi_{t}$ are:
\begin{equation}
\begin{split}
%&\xi_{s,i} = \mu_{s,i} + \Sigma_{st,i}(\Sigma_{t,i}^{-1}(\xi_{t}-\mu_{t,i}))\\
%&\Sigma_{s,i} = \Sigma_{s,i}-\Sigma_{st,i}(\Sigma_{t,i}^{-1}\Sigma_{ts,i}) 
&y = \sum_{m=1}^{m}\beta({x_{m}^{*}}) (\mu_{y}^{m}+\Sigma_{yx^{*}}^{m}(\Sigma^{m}_{x^{*}x^{*}})^{-1}(x^{*}-\mu^{x^{*}}_{m}))\\
&\Sigma = \beta({x_{m}^{*}})^2(\sum_{m=1}^{m}\Sigma^{m}_{yy}(\Sigma_{xx}^{m})^{-1}\Sigma_{xy}^{m})
    \end{split}
\end{equation}
where $\beta$ gives a relative importance of each Gaussian component. Then, the regression model $\{y,\Sigma\}$ is computed given $x^{*}$. Repeat this procedure for each necessary query point.

==> kde.tex <==
\gls{kde} is non-parametric method to estimate the \gls{pdf} of motion artifact $\ART$. This can be computed using
\begin{equation}
    \hat{f(\art)} = \frac{1}{nh} \sum_{i=1}^n k\bigg(\frac{\norm{\art-\art_i}}{h}\bigg),
\end{equation}
where $n$ is the sample size, $K(·)$ is standard normal distribution, $\art_i$ is motion artifiact, and $h$ is the bandwidth. The choice of bandwidth $h$ is using Silverman's rule. This is computed using 
\begin{equation}
    h = \sigma(\frac{4}{3n})^{\frac{1}{5}}
\end{equation}
where $\sigma$ is applying a robust estimator. The formula is following
\begin{equation}
\sigma = \frac{\text{Median}(\left|\art_i - \text{Median}(\art)\right|)}{0.6745}.
\end{equation}

\subsection{histogram}
The number of bin of the histogram is computed using square-root choice, which is computed by
\begin{equation}
k =\lceil \sqrt{n} \rceil = 81
\end{equation}

where $\tilde{f(x)}$ is estimated by histogram. This is computed by:
\begin{equation}
    \tilde{f(x)} = \frac{\text{number of observations within each bin}}{k*\text{binwidth}}
\end{equation}


\subsection{Goodness-of-fit evaluation}
\begin{equation}
\text{MSE} =  \frac{1}{k}\sum_{i=1}^{k} ( \hat{f(x)}-\tilde{f(x))}^2
\end{equation}
\subsection{Estimate \gls{mi} using \gls{kde}}
\gls{mi} between two difference movements could be estimated using \gls{kde} \cite{moon1995estimation}. (This is for muti-dimension data. One dimension case could be updated afterforwards.)
\begin{equation}
    \hat{\Prob}(\Df)=\frac{1}{n}\sum_{i=1}^{B}K(u),
\end{equation}
where
\begin{equation}
    u = \frac{(\xf-\xf{i})^\T S^{-1}(\xf-\xf{i})}{h^{2}},
\end{equation}
$K(u)$ is Gaussian kernel density function. $S$ is the covariance matrix on the $\Df_{i}$.
\gls{mi} between two movements $I(\Df_{\w1},\Df_{\w2})$ can be estimated by
\begin{equation}
I(\Df_{\w1},\Df_{\w2}) = \sum_{i,j}\Prob(\xf_{\w1}^{i},\xf_{\w2}^{j})\log_{2}\frac{\xf_{\w1}^{i},\xf_{\w2}^{j}}{\xf_{\w1}^{i}\xf_{\w2}^{j}}.
\end{equation}

==> related_work.tex <==
In this section, \note{\done{Use passive voice.}}{MH}\note{\done{Use present tense.}}{MH}relevant work in  fabric/clothing movement analysis and human motion trajectory forecasting is reviewed. From this, \note{\done{Use passive voice.}}{MH}\note{\done{Use present tense.}}{MH}the research gap and\note{Use present tense.}{MH} the main contributions of this paper are introduced. 

\subsection{Fabric/clothing movement analysis}\label{s:fabric_clothing_movement_analysis}%
In recent years, researchers have been investigating motion analysis using clothing-attached sensors. However, the most of work are comparing accuracy of \gls{ar} between using body and clothing-attached sensors. \textcite{michael2017} used a pendulum with a piece of fabric attached as the physical model and classify low and high swing speed using rigid and fabric-attached sensors. The results\note{\done{Check English/rephrase.}}{MH} suggest that fabric movement may actually \emph{assist} human motion analysis, particularly in \gls{ar}. \textcite{jayasinghe2019comparing} found that the movements of clothes can be useful for describing daily human activities, such as walking, running, sitting, and riding a bus and for gait analysis \cite{jayasinghe2022comparing}. \textcite{jayasinghe2023classification} also used loose fitting trousers-attached sensors to classify simple static postures (\ie standing, sitting, lying down and sitting on the floor) based on acceleration. Three features (inclination angles of the waist, thigh, and ankle) are used and three simple static postures are classified using \gls{knn} algorithm. The high accuracy indicates that using clothing-attached sensors to make a classification between completely different static postures is promising.\note{This is pretty suspicious. Do you really believe their classifier is perfect, \ie made no errors at all? (If so, what is the point of your work? If you can get perfect activity recognition from their approach, there seems little point in further study on the topic.) Perhaps they were only using simple movement data?}{MH} \textcite{hoareau2023evaluation} used clothing-attached sensors to detect trunk and upper arm postures and movements while the user was talking several work tasks.\note{\done{Check English/rephrase.}}{MH} The results show that the performance is task dependent and influenced by individual factors such as clothing fit. Given the balance between accuracy, comfort, and ease of use, clothing-attached sensors could be a hopeful choice. \textcite{airaksinen2020automatic} developed a sensor-embedded jumpsuit for infants for detecting and tracking infant movement activities using \gls{cnn} to identify infants who are vulnerable to a variety of neurodevelopmental problems. The findings of our previous work \cite{shen2022probabilistic} is the looser fabric can get better performance in \gls{ar}, particularly when classifying different frequencies of simple harmonic motion from short time windows. This verification was conducted through numerical simulations, as well as experiments involving simple harmonic motion and a hand crank. The probabilistic model was proposed to understand and explain this phenomenon. The explanation is motion artefacts can increase the statistical distance between different movements, thus simplifying the classification task. This probabilistic model also can be used to predict how performance of \gls{ar} between the body and clothing-attached sensor is increased. This work was also extended with more participants in hand crank experiment. The robustness of our findings can be enhanced by this. \note{\done{Use passive voice.}}{MH} Additionally, numerical calculations of the probabilistic model is provided \cite{shen2023probabilistic}.\note{You give far more description to your work than others: I suggest you reduce this and focus on the key points. In particular, you need to explain how/why this paper makes a different contribution to that one.}{MH}

As introduced above, the current research in fabric/clothing movement analysis is limited to \gls{ar} using loose clothing. For example, it includes classifying low and high swing speeds of pendulum, different static postures, \etc The performance of trajectory forecasting using loose clothing has not been explored and it is a greater challenge task.
\note{What is the conclusion from your survey of works in \sref{fabric_clothing_movement_analysis}? What is the gap you are filling?}{MH}
\note{It would be good to add intro/outro sentences to \sref{fabric_clothing_movement_analysis} to link it to the rest of the paper. It currently reads as a list of works with no clear message.}{MH}
\subsection{Human motion trajectory forecasting}\label{s:trajectory_forecasting}
Recently, many researchers also focus on human motion trajectory prediction and forecasting, particularly for the application of collaborative, production and rehabilitation robots. \textcite{liu2017human} used \gls{hmm} to predict the worker's future activity and generated an activity transition probability matrix. A skilled worker successfully collaborated with a robot arm to assemble a car engine.\note{\done{Check English/rephrase.}}{MH} The worker's movement was recorded by a RGB camera and the robot was able to predict the worker's activity sequence. The results show that the predicted human movements could be applied to task-level collaborative human-robot assembly. \textcite{chen2018wristcam} presented a wearable camera sensor tightly worn on the wrist used to detect the movement of hand trajectory gestures. They successfully applied to an application of controlling a collaborative robot to draw letters on paper. This demonstrates that a wearable camera sensor worn on the wrist could be practical in human-robot collaboration. \textcite{dinh2015approach} used a human motion prediction technique to prevent collisions in the context of \gls{hrc}. Participants were invited to Sort LEGO-bricks together with the robot concurrently operating within the shared workspace. The occurrence of a collision is possible and should be avoided. $4$ cameras were used to record human-robot positions and A human motion prediction algorithm based on the minimum-jerk model is developed to avoid collision. The assessment of the comfort and acceptance of the robot collaborator by the human collaborator is elicited via an analysis of subjective participants feedback questionnaires.

In addition to record human skeleton movements using camera, other types of information can be used to predict human motion, for example, \gls{imu}, \gls{emg}. \textcite{sirintuna2020detecting} collected \gls{emg} from human arm muscles to predict human motion intention using \gls{nn}. $6$ participants were invited to complete path following task collaborated with a robot arm. The results show this method can effectively support humans in task execution and the unintended motion errors is also low. \textcite{ren2019deep} used Myo armband tighly attached to the human arm. The Myo armband is a device embedded with \gls{imu} and \gls{emg} sensors. The wearer's future motion can be forcasted using deep learning method. Therefore, the robot arm is capable of real-time tracking the movements on either side of the wearer's arm. 

%Researchers in the field of computer vision are also interested in human motion prediction. 
As previously mentioned, the current research in human motion trajectory forecasting collects \gls{imu}s, \gls{emg} and human skeleton. Data acquisition device could include cameras and body-worn sensors. The clothing-attached sensors could be another choice, given the benefits of comfortable wearing and unobtrusive sensing. Furthermore, using clothing-attached sensors can get higher accuracy of \gls{ar} as discussed in our previous work \cite{shen2022probabilistic,shen2023probabilistic}. The performance of trajectory forecasting using clothing-attached sensors is valuable to be explored.
\note{The last two comments also apply to \sref{trajectory_forecasting}.}{MH}
\subsection{Distance between \gls{hmm}s}\label{s:distance}
Several research efforts have been made on estimating the distance between \gls{hmm}s. The pioneering study \cite{juang1985probabilistic} uses Monte Carlo simulation but experimental results on continuous \gls{lr-hmm} were not reported. The smiliar approach used for continuous \gls{lr-hmm} is reported in \cite{singh2000structured}. But, this method needs to generate ergodic Markov chains underlying \gls{hmm} parameter $\lambda$.%
\note{Check English/rephrase: Avoid starting sentences with ``But''.}{MH}%
Therefore, the result is highly dependent on the quality of the estimated \gls{hmm} parameter $\lambda$. One paper \cite{zhao2007measuring} proposes a method to estimate upper bound of a symmetric \gls{kl}. But, it is not appropriate to use since the element of transition matrix $\bA$ could be zero in \gls{lr-hmm}, which cannot be computed in logarithm. \textcite{huo2006dtw} used \gls{dtw}-based method to estimate distance between two \gls{lr-hmm}s. But, it is not appropriate to use in this paper as the sampling frequency of the sensor is not changed. Some methods consider all different state sequences \cite{hershey2008variational,hershey2007variational,jebara2007spectral}.

\subsection{Main contributions}
%However, the current research is limited to activity recognition using fabric motion. \note{\done{Check English/rephrase.}}{MH} The performance of trajectory forecasting using loose clothing has not been explored.\note{This is the gap you are filling, but it is not clear from the literature review that this gap exists. }{MH} On the other hand, most of the research work on trajectory forecasting by recording the movement of human skeletons.\note{If so, why is this work not discussed above?}{MH} They have not considered the possibility of using clothing motion. \note{Ditto.}{MH}
The following is a summary of this work's main contributions.
\begin{itemize}
  \item To the authors’ knowledge, this is the first paper using fabric movement to forecast the future trajectory.\note{\done{Use passive voice.}}{MH}\note{\done{Use present tense.}}{MH} The performance of trajectory forecasting using body and clothing-attached sensors is also compared.
%  \item We\note{Use passive voice.}{MH} proposed\note{Use present tense.}{MH} the probabilistic trajectory models and estimated\note{Use present tense.}{MH} the probabilistic distance between two activtity movements to understand this phenomenon.\note{Check English/rephrase.}{MH}
\end{itemize}

